Constant Weight Codes with Gabor Dictionaries and Bayesian Decoding for Massive Random Access

This paper considers a general framework for massive random access based on sparse superposition coding. We provide guidelines for the code design and propose the use of constant-weight codes in combination with a dictionary design based on Gabor frames. The decoder applies an extension of approximate message passing (AMP) by iteratively exchanging soft information between an AMP module that accounts for the dictionary structure, and a second inference module that utilizes the structure of the involved constant-weight code. We apply the encoding structure to (i) the unsourced random access setting, where all users employ a common dictionary, and (ii) to the "sourced" random access setting with user-specific dictionaries. When applied to a fading scenario, the communication scheme essentially operates non-coherently, as channel state information is required neither at the transmitter nor at the receiver. We observe that in regimes of practical interest, the proposed scheme compares favorably with state-of-the art schemes, in terms of the (per-user) energy-per-bit requirement, as well as the number of active users that can be simultaneously accommodated in the system. Importantly, this is achieved with a considerably smaller size of the transmitted codewords, potentially yielding lower latency and bandwidth occupancy, as well as lower implementation complexity.

==> sections/inference_old.tex <==
\section{Inner Decoder}\label{sec:appendix}
\begin{comment}
\subsection{Separate Dictionaries}
Consider the system model from Section \ref{sec:separate_dictionaries} for the scenario where the users use separate dictionaries for transmission, $\mathbf{y}=\ASD\mathbf{x}+\noise$. As described in Section~\ref{sec:separate_dictionaries}, this channel can be viewed as a concatenation of an inner channel $\mathbf{x}\rightarrow \mathbf{A}\mathbf{x}+\noise$, and a bank of parallel outer channels $(\mathbf{c}_{i_1}, \ldots,\mathbf{c}_{i_K})\rightarrow (\mathbf{x}_{i_1}, \ldots,\mathbf{x}_{i_K})$, where $\mathbf{c}_{i_1}, \ldots,\mathbf{c}_{i_K}$ are the binary codewords of the users that are active over a single resource block of $n$ channel uses. The structure of the code construction for this scenario admits an iterative Bayesian decoding procedure where at the receiver side soft information is exchanged between an inner and an outer decoder in an iterative (turbo-like) fashion. In the example when the constant weight (CW) code is obtained by concatenating a PPM code with an outer non-binary code (such as RS code in our construction), the inner decoder consists of an AMP Module that is modified to incorporate the decoding of the PPM code. The output of the inner decoder is input to the outer decoder for the non-binary outer code that provides sparsity update to the inner decoder by accounting for the structure present in the outer code. In our examples, for this step we rely on a soft-input-soft-output decoding algorithm for RS codes \cite{bimberg10}.  
\end{comment}
%\subsection{Inner Decoder}
In the following we present the details of the Bayesian inference procedure for the inner decoder. We describe the inference procedure for the extended system model with a single-antenna transmitters and a multi-antenna receiver (SIMO) with $T$ antenna elements in a block-fading scenario. The task of the inner decoder consists of detecting the transmitted sequences and is realized for both communication procedures, i.e., with separate and common dictionaries, using the same algorithmic solution. To be more specific, we use the MMV-AMP algorithm, which has been introduced in \cite{kim2011belief}. Let
\begin{equation}
    \mathbf{Y}=\mathbf{A}\mathbf{X}+\mathbf{W}
\end{equation}
be the general system model of the inner channel, with transmit matrix $\mathbf{X}\triangleq[\mathbf{x}_1,\dots,\mathbf{x}_N]^T\in\mathbb{C}^{N\times T}$, receiver noise matrix $\mathbf{W}\triangleq[\mathbf{w}_1,\dots,\mathbf{w}_n]^T\in\mathbb{C}^{n\times T}$ and measurement matrix $\mathbf{Y}\in\mathbb{C}^{n\times T}$. Regardless of the considered communication setup, the inner decoder considers the rows of $\mathbf{X}$ to be statistical independent. Let $\epsilon=\frac{\rho\Ktot}{M}$ be the fraction of active sequences with $\rho$ denoting the probability of user activation, the distribution of $\mathbf{X}$ is given by
\begin{equation}
    P_{\mathbf{x}}(\mathbf{x}_k)=(1-\epsilon)\delta(\mathbf{x}_k)+\epsilon P_{\mathbf{h}}(\mathbf{h}_k)\label{eq:prior}
\end{equation}
where $P_{\mathbf{h}}(\mathbf{h}_k)$ denotes the distribution of the block-fading channel, which for Rayleigh is defined as $P_{\mathbf{h}}(\mathbf{h}_k)=\mathcal{CN}(0,\mathbf{I})$.
With $\mathbf{X}^0=0$ and $\mathbf{Z}^0=\mathbf{Y}$, the iterations of MMV-AMP are given by
\begin{align}
    \tau_{t+1,i}^2&=\Vert\mathbf{Z}^t\Vert^2_2\\
    \mathbf{X}^{t+1}&=\eta(\mathbf{A}^{\mathrm{H}}\mathbf{Z}^t+\mathbf{X}^t,\boldsymbol{\tau}_{t+1})\\
    \mathbf{Z}^{t+1}&=\mathbf{Y}-\mathbf{A}\mathbf{X}^{t+1}+\frac{N}{n}\mathbf{Z}^t\langle \eta'(\mathbf{A}^{\mathrm{H}}\mathbf{Z}^t+\mathbf{X}^t,\boldsymbol{\tau}_{t+1})\rangle\label{eq:eta_prime}
\end{align}
The non-linear denoising function $\eta:\mathbb{C}^{N\times T}\times \mathbb{R}^T\rightarrow \mathbb{C}^{n\times T}$ defined as
\begin{equation}
    \eta(\mathbf{R},\boldsymbol{\tau}):=[\eta_1(\mathbf{R}_1,\boldsymbol{\tau}_1),\ldots,\eta_N(\mathbf{R}_{N},\boldsymbol{\tau}_N)]^{\mathrm{T}}
\end{equation}
where the row-wise denoising function $\eta_k:\mathbb{C}^T\times \mathbb{R}^T$ computes the posterior mean estimate of the random vector $\mathbf{x}_k$, with prior distribution defined in \eqref{eq:prior} and the decoupled Gaussian likelihood assumption 
\begin{equation}
    \mathbf{R}_k=\mathbf{X}_k+\mathbf{Z}_k\label{eq:noisy_decoupled}
\end{equation}
with $\mathbf{z}_k\sim\mathcal{CN}(\boldsymbol{0},\mathrm{diag}(\boldsymbol{\tau}))$. The posterior mean is defined by
\begin{equation}
    \eta_k(\mathbf{r}_k,\boldsymbol{\tau}):=\mathbb{E}[\mathbf{x}_k\vert \mathbf{r}_k,\boldsymbol{\tau}].
\end{equation}
which for Rayleigh fading becomes
\begin{equation}
     \eta_k(\mathbf{R}_k,\boldsymbol{\tau})=\phi(\mathbf{R}_k,\boldsymbol{\tau}_k)(\mathbf{I}+\Sigma_k)^{-1}\mathbf{R}_k
\end{equation}
with
\begin{equation}
    \phi(\mathbf{R}_k,\boldsymbol{\tau}_k)=\left(1+\frac{(1-\epsilon)}{\epsilon}\frac{\vert\mathbf{I}+\Sigma_k\vert}{\vert\Sigma_k\vert}\exp(-\mathbf{R}_k^{H}\tilde{\Sigma}_k^{-1}\mathbf{R}_k)\right)^{-1}
\end{equation}
where we defined $\Sigma_k=\mathrm{diag}(\boldsymbol{\tau}_k)$ and $\tilde{\Sigma}_k=\Sigma_k\Breve{\Sigma}_k$ with $\Breve{\Sigma}_k=\mathbf{I}+\Sigma_k$. The term $\eta'(\cdot,\cdot)$ in \eqref{eq:eta_prime} is defined by the Jacobi 

\begin{multline}
    \eta'(\mathbf{r}_k,\boldsymbol{\tau})=\\
    \phi(\mathbf{r}_k,\boldsymbol{\tau}_k) \tilde{\Sigma}_k^{-1} + (\Breve{\Sigma}_k^{-1}\mathbf{R}_k)(\tilde{\Sigma}_k^{-1}\mathbf{R}_k)^H(\phi(\mathbf{R}_k,\boldsymbol{\tau}_k)-\phi(\mathbf{R}_k,\boldsymbol{\tau}_k)^2)
\end{multline}


%\begin{figure}[h]
%\resizebox{.9\linewidth}{!}{\input{tikz/factorgraph.tex}}
%\caption{Factor graph for separate dictionary setup.}
%\label{fig:graph_model}
%\end{figure}

\section{User Activity Detection with Separate Dictionaries}\label{sec:AD}
%: With this, the inference procedure in general may be formulated as a joint estimation problem of the binary code vector $\mathbf{c}\triangleq[\mathbf{c}_1;\dots;\mathbf{c}_L]\in\{0,1\}^{NL}$, and the channel matrix $\mathbf{X}\triangleq[\mathbf{x}_1,\dots,\mathbf{x}_L]^T\in\mathbb{C}^{NL\times T}$, given the measurements matrix $\mathbf{Y}\in\mathbb{C}^{n\times T}$. The Bayesian treatment of the inference problem requires the formulation of a joint posterior distribution over all random variables, given by
%\begin{multline}
%    P(\mathbf{c},\boldsymbol{\lambda},\mathbf{x}\vert\mathbf{y}) = P(\mathbf{y}\vert\mathbf{z})P(\mathbf{y}|\mathbf{c})P(\mathbf{c}|\boldsymbol{\lambda})P(\boldsymbol{\lambda})/P(\mathbf{y})\\
%    \propto P(\mathbf{y}\vert\mathbf{z})\prod\limits_{l}P(\mathbf{x}_l\vert\mathbf{c}_l)P(\mathbf{c}_l|\lambda_l)P(\lambda_l)\label{eq:joint}  
%\end{multline}
%with $\mathbf{z}=\ASD \mathbf{x}$. The users are assumed to be independently active with probability $ P(\lambda_l=1)=\rho_l$. Under the assumption of additive Gaussian measurement noise at the receiver the likelihood of the measurement matrix $\mathbf{y}$ in \eqref{eq:joint} reads
%\begin{equation}
%    P(\mathbf{y}\vert\mathbf{z})=\mathcal{CN}(\boldsymbol{0}, N_0\mathbf{I}).
%\end{equation}
%Further we define
%\begin{equation}
%    P(x_j|c_j)=c_jP(h_j)+(1-c_j)\delta(x_j)\label{eq:prior1}
%\end{equation}
%where $P(h_j)$ is the statistical distribution of the block-fading channel.


Assuming that every user uses the previously introduce constant weight construction given by $\mathcal{C}_{\mathrm{CW}}=\mathrm{PPM}(M)\circ \mathrm{RS}(N,k)$ to encode its message and under the assumption of equiprobable messages, the pdf of the message vector $\mathbf{c}_l=[\mathbf{c}_l^{(1)};\ldots;\mathbf{c}_l^{(N)}]$ given the user activity variable $\lambda_l$ is given by
\begin{equation}
    P(\mathbf{c}_l\vert\lambda_l)=\prod_{n=1}^N P(\mathbf{c}_l^{(n)}\vert\lambda_l)
\end{equation}
with for every sub-vector $\mathbf{c}_l^{(n)}$ we have
\begin{equation}
    P(\mathbf{c}_l^{(n)}\vert\lambda_l)=\begin{cases}
        \frac{1}{M}\sum\limits_{j=1}^{M}\delta(c_{jl}^{(n)}-1)\prod\limits_{k\neq j}^{M}\delta(c_{kl}^{(n)})&\mathrm{for } \lambda_l=1\\
        \prod\limits_{j=1}^{M}\delta(c_j) &\mathrm{for } \lambda_l=0.
    \end{cases}\label{eq:prior4}
\end{equation}
where we use $c_{kl}^{(n)}$ to denote the $k$th element of $\mathbf{c}_l^{(n)}$.
The goal of the inner decoder is it to jointly detect the active users and their corresponding binary CW codes $\{\lambda_l,\mathbf{c}_l\}_{l=1}^L$ from the noisy observations $\mathbf{y}$ given the separate dictionaries $\ASD$ and the statistical information on $\lambda_l,\mathbf{c}_l,h_l$ and $\mathbf{w}$. As we intend to iterate in a turbo-like fashion between the inner decoder and an outer soft-input-soft-output decoder, we are interested in the posterior distribution of the detected CW code entries given by
\begin{equation}
    P(c_{lj}^{(n)}\vert \mathbf{y})=\sum_{\mathbf{c}/c_{lj}^{(n)}}\sum_{\boldsymbol{\lambda}/\lambda_l}\int_{d\mathbf{x}}P(\mathbf{x},\mathbf{c},\boldsymbol{\lambda}\vert\mathbf{y}).\label{eq:posterior_marginal}
\end{equation}

With the the likelihood assumption from \eqref{eq:noisy_decoupled} the likelihood distribution for the outer factor graph is given by
\begin{equation}
    P(\mathbf{x}_k|\mathbf{r}_k)=\mathcal{CN}(\mathbf{r}_k,\Theta)[(1-\lambda)\delta(\mathbf{x}_k)+\lambda P_{\mathbf{h}}(\mathbf{h}_k)]
\end{equation}

\subsubsection*{User Activity}
The rightwards message from the user the message prior $f_{\mathbf{c}}(\lambda)$ to user activity $\lambda$ is given by
\begin{equation}
    \nu_{f_{\mathbf{c}}\rightarrow\lambda}(t,\lambda)\propto
    \sum_{\mathbf{c}\in\mathcal{C}}f_{\mathbf{c}}(\mathbf{c}|\lambda)\prod_{j=1}^N\nu_{c_j\rightarrow f_{\mathbf{c}}}(t,c_j)
\end{equation}
and after marginalization we have
\begin{multline}
    \nu_{f_{\mathbf{c}}\rightarrow\lambda}^{(n)}(t,\lambda_l)\propto\\
    \begin{cases}
        \frac{1}{M}\sum_j\nu_{c_{j}\rightarrow f_{\mathbf{c}}}^{(n)}(t,1)\prod_{i\neq j}\nu_{c_i\rightarrow f_{\mathbf{c}}}^{(n)}(t,0)&, \lambda_l=1\\
        \prod_{j}\nu_{c_{j}\rightarrow f_{\mathbf{c}}}^{(n)}(t,0) &, \lambda_l=0
    \end{cases}
\end{multline}
which 
\begin{equation}
    \mathrm{LLR}_{f_{\mathbf{c}}\rightarrow\lambda}^{(n)}(t)=\log \sum_{j}\frac{\nu^{(n)}_{c_{j}\rightarrow f_{\mathbf{c}}}(t,1)}{\nu^{(n)}_{c_{j}\rightarrow f_{\mathbf{c}}}(t,0)}-\log M
\end{equation}

\begin{equation}
    \mathrm{LLR}_{\lambda}(t+1)=\sum_n\mathrm{LLR}_{f_{\mathbf{c}}\rightarrow\lambda}^{(n)}(t)+\log \rho_l/(1-\rho_l)
\end{equation}
and 
\begin{equation}
    \hat{\rho}_l(t+1)\triangleq (1+\exp -\mathrm{LLR}_{\lambda}(t+1))^{-1}
\end{equation}
\subsubsection*{Message variables}
The leftward message update from $f_{\mathbf{c}}$ to $\mathbf{c}$ is given by
\begin{multline}    
    \nu_{f_{\mathbf{c}}\rightarrow c_j}(t,c_j)\propto\\
    \sum_{\lambda_l}\nu_{\lambda\rightarrow f_{\mathbf{c}}}(t,\lambda_l)\sum_{\mathbf{c}/c_j}f_{\mathbf{c}}^{(n)}\prod_{i\neq j}\nu_{c_i\rightarrow f_{\mathbf{c}}}(t,c_i)
\end{multline}
after marginalization we get
\begin{multline}
    \nu_{f_{\mathbf{c}}\rightarrow c_j}(t,c_j)\propto\\
    \begin{cases}
    \frac{\hat{\rho}_l^t}{M}\nu_{c_j\rightarrow f_{\mathbf{c}}}(t,1)\prod\limits_{i\neq j}\nu_{c_i\rightarrow f_{\mathbf{c}}}(t,0)  &,\, c_j=1\\
    \frac{\hat{\rho}_l^t(M-1)}{M}\sum\limits_{i\neq j}\nu_{c_i\rightarrow f_{\mathbf{c}}}(t,1)\prod\limits_{k\neq i}\nu_{c_k\rightarrow f_{\mathbf{c}}}(t,0)&\\
    +(1-\hat{\rho}_l^t)\prod\limits_{k}\nu_{c_k\rightarrow  f_{\mathbf{c}}}^t(0) &,\, c_j = 0
    \end{cases}
\end{multline}
which leads to following LLRs
\begin{multline}    
\mathrm{LLR}_{f_{\mathbf{c}}\rightarrow c_{lj}}^t=\\
\frac{\nu_{c_j\rightarrow f_{\mathbf{c}}}(t,0)}{\nu_{c_j\rightarrow f_{\mathbf{c}}}(t,1)}\left((M-1)\sum\limits_{i\neq j}\frac{\nu_{c_i\rightarrow f_{\mathbf{c}}}(t,1)}{\nu_{c_i\rightarrow f_{\mathbf{c}}}(t,0)}+\frac{M(1-\hat{\rho}_l^t)}{\hat{\rho}_l^t}\right)\label{lr1}
\end{multline}
and for the subsequent derivations we also introduce following variable
\begin{equation}
    \hat{\epsilon}_{lj}^{t+1}=(1+\exp(-\mathrm{LLR}_{f_{\mathbf{c}}\rightarrow c_{lj}}^t))^{-1}\label{epsilon}
\end{equation}


\begin{comment}
The computation of the marginals in \eqref{eq:posterior_marginal} is intractable due to the coupling of $\mathbf{x}$ and $\mathbf{z}$ through the dense dictionary matrix $\ASD$. Approximate solutions to \eqref{eq:posterior_marginal} can however be computed via message passing algorithms (also known as belief propagation (BP)), which exploit the \textit{factorizable} structure of \eqref{eq:joint} to reduce the computational complexity. The factorization of \eqref{eq:joint} is well illustrated using a factor graph representation. The graphical model corresponding to \eqref{eq:joint} is depicted in Fig.~\ref{fig:graph_model}. Factors are represented using filled squares, and random variables using circles.
The factorization in \eqref{eq:joint} can be encoded in a factor graph $G=(V,F,E)$, where $V$ is the set of variable nodes, $F$ is the set of factor nodes and $E$ denotes the set of edges. 
\subsubsection*{Approximate Message Passing} 
Using a dense sensing matrix $\mathbf{A}$, makes the problem even with belief propagation intractable. Approximate message passing has been introduced as an approximation for the message updates for linear inverse problems \cite{Donoho}. The standard AMP algorithm, as originally introduced in \cite{Donoho}, considers the estimation of a vector $\mathbf{x}$ with independent components and additive Gaussian noise. In order to allow for noise models other than Gaussian, the so-called generalized-AMP (GAMP) has been introduced in \cite{Rangan11}. In order to introduce correlations and structural dependencies of the input variables, a hybrid extension of the AMP algorithms has been introduced in \cite{rangan17}. This extension of AMP allows a systematic treatment of correlations between variables into the AMP algorithm. %The message updates for the joint user activity and message detection are listed in Algorithm~\ref{alg:gamp}. 
The messages will be derived in the following.
\end{comment}

\begin{algorithm}[h]
\caption{Inner decoder}\label{alg:gamp}
\begin{algorithmic}[1]
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\REQUIRE $\mathbf{y}$, $\mathbf{A}$
\STATE \{Initialization\}
\STATE \{Outer Loop\}
\FOR {$l=1$ to $L_{\mathrm{Max}}$} 
\STATE \{Inner Decoding with MMV-AMP\}
\FOR {$t=1$ to $T_{\mathrm{Max}}$} 
\STATE $\hat{x}_{j}^{t}= \mathbb{E}[x_{j}\vert\hat{r}_{j}(t-1),v_{j}^{r}(t-1),\hat{\epsilon}_{j}(t-1)]$\label{step1} see \ref{mmse1}
\STATE $v_{j}^{x}(t)=\mathrm{var}[x_{j}\vert\hat{r}_{j}(t-1),v_{j}^{r}(t-1),\hat{\epsilon}_{j}(t-1)]$\label{step2}  see \ref{mmse2}
\STATE $v_{i}^{p}(t)= \sum_{j}\vert \mathbf{A}_{ij}\vert^2v^{x}_{j}(t)$
\STATE $\hat{p}_i(t)= \sum_{j} \mathbf{A}_{ij}\hat{x}_{j}(t)-v^{p}_i(t)\hat{s}_i(t-1)$
\STATE $\hat{z}_i(t)=(y_i-\hat{p}_i(t)(\sigma^2+v_i^{p}(t))^{-1}$
\STATE $v^{z}_i(t)=v_i^{p}(t)\sigma^2(\sigma^2 + v_i^{p}(t))^{-1}$ 
\STATE $\hat{s}_i(t)=(\hat{z}_i-\hat{p}_i(t))/v^{p}_i(t)$
\STATE $v_i^{s}(t)= (1-v_i^{z}(t)/v_i^{p}(t))/v_i^{p}(t)$
\STATE $v_{j}^{r}(t)=(\sum_{i}\vert\mathbf{A}_{ij}\vert^{2}v_{i}^{s}(t))^{-1}$
\STATE $\hat{r}_{j}(t)=\hat{x}_{j}^{t}+v_{j}^{r}(t)\sum_{i}\mathbf{A}^*_{ij}\hat{s}_{i}$
\ENDFOR
\STATE \{Updates for joint UA and Message detection\}
\STATE $\hat{\rho}_l(t+1)\leftarrow$\eqref{llr1}
\STATE $\hat{\epsilon}_{jl}^{(n)}(t)\leftarrow$\eqref{epsilon}
\STATE \{Update SISO\}
\STATE $\hat{\epsilon}_{jl}^{(n)}(t)\rightarrow\mathrm{SISO Decoder}$ 
\STATE $\hat{\epsilon}_{jl}^{(n)}(t+1)\leftarrow\mathrm{SISO Decoder}$ 
\ENDFOR
\end{algorithmic}
\end{algorithm}

%\subsubsection*{Derivation of HyGAMP Message Updates}
%To ease notation and readability in the following derivation we introduce following notation to denote factors, $h_l(\lambda_l)\triangleq p(\lambda_l)$, $   s_l(\mathbf{c}_l|\lambda_l)\triangleq p(\mathbf{c}_l|\lambda_l)$, $  f_{lj}(\mathbf{x}_{lj}|c_{lj})\triangleq p(\mathbf{x}_{lj}|c_{lj})$ and $   g_n(\mathbf{y}_n|\mathbf{z}_{n})\triangleq p(\mathbf{y}_n|\mathbf{z}_{n})$. Message from a variable $v$ to a factor $f$ will be denoted by $\nu_{v\rightarrow f}(v)$, the inverse messages by $\nu_{v\rightarrow f}(v)$. For binary variables we also define messages as log-likelihood-ratios (LLRs) given by $\text{LLR}_{v\rightarrow f}\triangleq\log\nu_{v\rightarrow f}(1)-\log\nu_{v\rightarrow f}(0)$ and likelihood-ratios by $\text{LR}_{v\rightarrow f}\triangleq\nu_{v\rightarrow f}(1)/\nu_{v\rightarrow f}(0)$.

\begin{comment}
\subsubsection*{Channel Variables}
The leftward message update from $f_{lj}(\mathbf{x}_{lj},c_{lj})$ to $\mathbf{x}_{lj}$ is given by
\begin{align}
    \nu_{f_{lj}\rightarrow\mathbf{x}_{lj}}^t(\mathbf{x}_{lj})&\propto\sum_{c_{lj}=0}^1 f_{lj}(\mathbf{x}_{lj},c_{lj}) \nu_{c_{lj}\rightarrow\mathbf{f}_{lj}}^t(c_{lj})
\end{align}
with marginalization leading to the Bernoulli-Gaussian distribution
\begin{align}
    \nu_{f_{lj}\rightarrow\mathbf{x}_{lj}}^t(\mathbf{x}_{lj})&\propto(1-\hat{\epsilon}_{lj}^t)\delta(\mathbf{x}_{lj})+\hat{\epsilon}_{lj}^t \mathcal{CN}(\mathbf{x}_{lj};0,\Sigma_l^h)
\end{align}
Using this distribution we can now compute step \ref{step1} and \ref{step2} of Algorithm~\ref{alg:gamp} given by
\begin{align}
\hat{\mathbf{x}}_{lj}^t&=\mathbb{E}\big[\mathbf{x}_{lj}\vert\hat{\mathbf{r}}_{lj}^t,\Sigma_{lj}^{r,t},\hat{\epsilon}_{lj}^t\big]\\
\Sigma_{lj}^{x,t}&=\text{var}\big[\mathbf{x}_{lj}\vert\hat{r}_{lj}^t,\Sigma_{lj}^{r,t},\hat{\epsilon}_{lj}^t\big]
\end{align}
with $\hat{r}_{lj}^t\sim\mathcal{CN}\big(\hat{r}_{lj}^t;\mathbf{x}_{lj}^t,\Sigma_{lj}^{r,t}\big)$. After some manipulation we get
\begin{align}
    \hat{\mathbf{x}}_{lj}&=\mathbf{t}_{lj}\mathbf{w}_{lj}\label{mmse1}\\
    \Sigma_{lj}^x&=\mathbf{t}_{lj}(1-\mathbf{t}_{lj})\mathbf{w}_{lj}^H+\mathbf{t}_{lj}((\Sigma_{lj}^x)^{-1}+(\Sigma_{lj}^r)^{-1})^{-1}\label{mmse2}
\end{align}
with
\begin{align}
    \mathbf{w}_{lj}&=((\Sigma_{l}^h)^{-1}+(\Sigma_{lj}^r)^{-1})^{-1}(\Sigma_{lj}^r)^{-1}\hat{r}_{lj}\\
    \mathbf{t}_{lj}&=\left(1+\frac{1-\hat{\epsilon}_{lj}}{\hat{\epsilon}_{lj}}\vert\Sigma_{lj}^r+\Sigma_{l}^h\vert/\vert\Sigma_{lj}^r\vert\exp\left(-\hat{\mathbf{r}}_{lj}^H\Gamma_{lj}\hat{\mathbf{r}}_{lj}\right)\right)^{-1}
\end{align}
where $\vert\Sigma_{lj}^r\vert$ and $\vert\Sigma_{lj}^r+\Sigma_{l}^h\vert$ are the determinants of the respective covariance matrices and with $\Gamma_{lj}\triangleq((\Sigma^r_{lj})^{-1}-(\Sigma^r_{lj}+\Sigma^x_{lj})^{-1})$. 

The rightwards message updates from $\mathbf{x}_{lj}$ to $f_{lj}(\mathbf{x}_{lj},c_{lj})$ is given by
\begin{equation}
    \nu_{\mathbf{x}_{lj}\rightarrow f_{lj}}^t(\mathbf{x}_{lj})\propto \mathcal{CN}\big(\hat{r}_{lj}^t;\mathbf{x}_{lj}^t,\Sigma_{lj}^{r,t}\big)
\end{equation}
and the rightward messages from $f_{lj}(\mathbf{x}_{lj},c_{lj})$ to $c_{lj}$ are given by
\begin{equation}
    \nu_{f_{lj}\rightarrow c_{lj}}(c_{lj})\propto \int f_{lj}(\mathbf{x}_{lj},c_{lj}) \mathcal{CN}\big(\hat{r}_{lj}^t;\mathbf{x}_{lj}^t,\Sigma_{lj}^{r,t}\big) d\mathbf{x}_{lj}
\end{equation}
which leads to 
\begin{multline}
    \text{LR}_{f_{lj}\rightarrow c_{lj}}^t=\frac{\hat{\epsilon}_{lj}^t}{(1-\hat{\epsilon}_{lj}^t)}\frac{\vert\Sigma_{lj}^{r,t}\vert}{\vert\Sigma_{lj}^{r,t}+\Sigma_{l}^{h,t}\vert}\exp\left(\hat{\mathbf{r}}_{lj}^{H,t}\Gamma_{lj}^t\hat{\mathbf{r}}_{lj}^t\right)\label{llr1}
\end{multline}
and $\text{LR}_{f_{lj}\rightarrow c_{lj}}^t\triangleq\text{LR}_{c_{lj}\rightarrow s_l}^t$ can then be inserted in \ref{lr1}.
\end{comment}

\subsection*{Outer decoder}
In order to accommodate the iterative decoding of the CW code in the Hybrid AMP inference framework, we need a soft-input soft-output (SISO) decoding algorithm that will take as input the soft information obtained from the outer decoder, and output soft information (sparsity update) to the inner decoder in an iterative procedure. For the case when the outer code is an RS code, we rely on the SISO decoding algorithm from \cite{bimberg10} that performs non-binary adaptive belief propagation (GF-ABP). The approach can also be extended to perform multiple-bases belief propagation (GF-MBBP) that is suitable for
efficient parallel implementations. For more details of the algorithm we refer to \cite{bimberg10}.  

\begin{comment}
\subsection{Common Dictionary}

Consider the system model from Section \ref{sec:common_dictionary} for the scenario where the users use a common (shared) dictionary for transmission. In that case, the received signal can be written as $\mathbf{y}=\ASD\mathbf{x}+\noise$. 
%where, we recall, $\mathbf{y}=\left[\mathbf{y}_1; \ldots ; \mathbf{y}_{\rho}\right]\in \mathbb{C}^{\bar{n}\rho}$ stacks the signal vectors received over the $\rho$ blocks; $\mathbf{A}\in \mathbb{C}^{\bar{n}\rho\times N\rho}$ is a block diagonal matrix where each block contains the common dictionary matrix $\bar{\mathbf{A}}\in\mathbb{C}^{\bar{n}\times N}$; $\mathbf{x}=\left[\mathbf{x}_1;\ldots; \mathbf{x}_{\rho} \right]\in\mathbb{C}^{ N\rho\times 1}$, where $\mathbf{x}_r=\sum_{j=1}^K h_{ij}^{(r)}\mathbf{c}_{ij}^{(r)}$, for $r=1,\ldots,\rho$; and $\mathbf{z}=\left[\mathbf{z}_1; \ldots; \mathbf{z}_{\rho}\right]\in \mathbb{C}^{\bar{n}\rho\times 1}$ stacks the $\rho$ noise vectors. 
As discussed, this channel can be viewed as a concatenation of an inner channel $\mathbf{x}\rightarrow \ASD\mathbf{x}+\noise$, and an outer multiple access channel $(\mathbf{c}_{i_1}, \ldots,\mathbf{c}_{i_K})\rightarrow \mathbf{x}$, where $\mathbf{c}_{i_1}, \ldots,\mathbf{c}_{i_K}$ are the binary codewords of the users that are active over a single resource block.
    
As discussed in Section \ref{sec:decoding}, with this representation the decoding procedure may be formulated as a  concatenation of an inner and outer decoder. The inner decoder carries out AMP by treating the entries of the vector $\mathbf{x}$ as independent, and outputs soft information in the form of log-likelihood ratios for the entries of the support of $\mathbf{x}$. The outer decoder takes this soft information as input and outputs a list of $K$ codewords from the employed code $\mathcal{C}$ corresponding to the $K$ users active over the $\rho$ resource blocks ($K_a$ active users in total over all $V$ resource blocks, i.e. $n$ channel resources). We recall that, in the presented examples, we have considered $\mathcal{C}$ to be a constant weight code obtained by a (appropriately parameterized) concatenation of a PPM code and a Reed-Solomon code.  

As in the scenario with separate dictionaries, in the following we describe the inference procedure for the extended system model with a single-antenna transmitters and a  multiantenna receiver with $T$ antenna elements in a block-fading scenario. Again, for simplicity of the exposition, in the following we consider the scenario where the users transmit their messages over a single resource block ($\rho=1$) of size $\bar{n}$ channel uses, with the note that the extension to $\rho>1$ is straightforward, as the users apply the same dictionary over each resource block. With this, the inference procedure in general may be formulated as a joint estimation problem of the  binary codewords $\mathbf{c}_{i_1}, \ldots,\mathbf{c}_{i_K}$  and the matrix $\mathbf{X}\in\mathbb{C}^{N\times T}$ that stacks the $T$ (channel) vectors $\mathbf{x}$ (corresponding to the $T$ receive antennas)), given the measurements matrix $\mathbf{Y}\in\mathbb{C}^{n\times T}$. As before, we note that the inference procedure incorporates the AWGN scenario with a single-antenna receiver as a special case.

\subsubsection*{Inner decoder}    
For the inner decoder in this scenario, due to the independence of the user messages, the AMP formulation is just "plain" AMP with independent input variables and a sparsity rate $\epsilon_{j} = \frac{K w}{N}$  
where, we recall, $K$ is the number of users active over the resource block of length $n$ channel uses, $w$ is the weight of the CW code obtained by concatenating a PPM code and a Reed-Solomon code (as described in Section \ref{sec:Code_Design}), and $N$ is the dictionary size (which is equal to the block-length of the CW code). The definition of the update messages for the AMP algorithm with common dictionary are given in Algorithm~\ref{alg:gamp}.
\end{comment}

\section{Details on Constant Weight Decoding}\label{sec:appendix_outer_decoder}
The task of the outer decoder is to retrieve the the binary codewords of the users that are active over the $\rho$ resource blocks, $\mathbf{c}_{i_1}, \ldots,\mathbf{c}_{i_K}$, from the output of the inner decoder. The decoding is based on the procedure in \cite{AbdulJabbar88} for decoding of superimposed codes over multiaccess OR channels. There, the task is to map the binary superimposed sequence $\mathrm{f}(\mathcal{A})$ formed by the multiaccess OR channel into a set of codewords $\mathcal{A}=\{c_i\in\mathcal{C},\: i=1, \ldots, K\}$ from a given superimposed code $\mathcal{C}$. Let $\hat{\mathcal{A}}$ denote the decoder output set. Decoding was successful if the  set $\hat{\mathcal{A}}$ equals the transmitted set $\mathcal{A}$. 

Let $\mathrm{f}(\mathcal{A})$ be the superposition of a set $\mathcal{A}$ of codewords from a CW code $\mathcal{C}\in\mathcal{CW}\left(n,m,w,d\right)$ obtained by concatenating a PPM($q$) code with a systematic RS(n,k) code. The binary sequence $\mathrm{f}(\mathcal{A})$ can be written in a matrix form as a $\mathrm{q}\times \mathrm{n}$ binary matrix
\begin{equation}
   \mathrm{f}(\mathcal{A})=\begin{bmatrix}
\mathrm{f}_{01}       &  \mathrm{f}_{02}       & \dots     &  \mathrm{f}_{0\mathrm{n}}       \\
\mathrm{f}_{11}        &   \mathrm{f}_{12}       & \dots     &   \mathrm{f}_{1\mathrm{n}}       \\
\vdots  &  \vdots   &   \vdots  &   \vdots  \\   
\mathrm{f}_{(\mathrm{q}-1)1}       &   \mathrm{f}_{(\mathrm{q}-1)2}       & \dots     &   \mathrm{f}_{(\mathrm{q}-1)\mathrm{n}}       \\
            \end{bmatrix},\,\,\mathrm{ij}\in\{0,1\}.
\end{equation}
Let $S_j(\mathrm{f}(\mathcal{A}))$ denote the set of $\mathrm{GF}(q)$ symbols defined by the mapping
\begin{equation}
    S_j(\mathrm{f}(\mathcal{A}))=\left\{i\in\mathrm{GF}(q)\mid\mathrm{f}_{ij}=1\right\},\quad j\in[n],
\end{equation}
and $\mathrm{G}_{RS}$ denote the generator matrix of a systematic RS code over $\mathrm{GF}(q)$. Let further $B(\mathrm{f}(\mathcal{A}))$ denote a set of codewords from the code $\mathcal{C}$ defined by
\begin{equation}
    B(\mathrm{f}(\mathcal{A}))=\left\{\mathbf{F}\left(\mathrm{G}_{RS}\cdot\mathbf{i}\right)|\mathbf{i}=(\mathrm{i}_1,\mathrm{i}_2,\dots,\mathrm{i}_k), \,\,\mathrm{i}_l\in S_j(\mathrm{f}(\mathcal{A}))\right\},
\end{equation}
where $\mathbf{F}(\mathbf{c}_{RS})$ denotes the transformation from the RS codeword into a PPM(q) codeword. The decoder for the outer code can then be defined as the search procedure that produces following set of codewords
\begin{equation}
    \hat{\mathcal{A}}=\left\{\mathbf{c}\in B(\mathrm{f}(\mathcal{A}))\mid \langle\mathbf{c},\mathrm{f}(\mathcal{A})\rangle=w\right\}.
\end{equation}
The decoding complexity of the search decoder is equal to
\begin{equation}
    \mathrm{DC}(\mathrm{f}(\mathcal{A}))=|S_1(\mathrm{f}(\mathcal{A}))|\cdot |S_2(\mathrm{f}(\mathcal{A}))|\cdot \dots\cdot |S_k(\mathrm{f}(\mathcal{A}))|.
\end{equation}
Assuming $K$ active users over the resource block, the decoding complexity is upper bounded by
\begin{equation}
    \mathrm{DC}(\mathrm{f}(\mathcal{A}))\leq K^k.
\end{equation}
We note that the decoding complexity can be reduced by applying a form of Viterbi/trellis decoding based on the (soft) output of the inner AMP decoder coming in the form of log-likelihood ratios for the "active" sequences of the applied dictionary matrix.  

==> sections/results_old.tex <==
\section{Numerical Simulations}

In the following we give a numerical evaluation of the proposed communication schemes from Section~\ref{sec:system_model}. Following the evaluation procedure from \cite{polyanskiy17}, we consider a setup in which $\Ka$ active users from a pool of $\Ktot$ users simultaneously transmit messages of $b$ information bits over $n$ channel uses. Given the per-user constraint $E_s= n P$, the performance of the system is measured in terms of $\frac{E_b}{N_0}\doteq \frac{E_s}{b N_0}=\frac{\mathrm{SNR}}{b}$ required to serve the $\Ka$ active users with a fixed target error tolerance of $P_e\leq \epsilon$ defined in \eqref{eq:decoding_error_JC}. To compare against the results from, e.g., \cite{polyanskiy17,Fengler}, we evaluate our results against an effective number of channel uses of $\ntot=30000$, messages of $b=100$ information bits and a fixed message error probability of $P_e\leq 0.05$.

%As described in Section~\ref{sec:system_model}, we consider that the communication is performed over $n$ channel uses (channel resources) in total. There are $\Ktot$ users in the system that can transmit over the $n$ channel uses. Each active user transmits its codewords (packets) of size $n$ over a block. 
%In an OFDM-based system, for example, the above blocks could correspond to resource blocks (RBs), where each RB consists of $n_o$ OFDM symbols, each one spanning $n_{sc}$ consecutive subcarriers. Hence, an RB contains a total of $\bar{n} = n_o n_{sc}$ resource elements, and the packet length is $\rho n_o n_{sc}$. If the RBs are spread in frequency direction, then $n_o$ is related to the packet duration, whereas $\rho n_{sc}$ is related to the bandwidth ocuupancy. 
%In the simulations, we fix the error tolerance to $P_e\leq \epsilon$, and the message size (number of information bits) to $b$. Given the per-user constraint $E_s= n P$, the performance of the system is measured in terms of $\frac{E_b}{N_0}\doteq \frac{E_s}{b N_0}=\frac{\mathrm{SNR}}{b}$.

\subsection{Common Dictionary}
%In the following, we present selected numerical results for the approach when the users apply a common dictionary. Following the evaluation procedure from \cite{polyanskiy17}, we evaluate our results against an effective number of channel uses of $\ntot=30000$ and a fixed message error probability of $P_e\leq 0.05$. 
%We recall that, although the random access model is unsourced, in the case when the active users spread their messages over $\rho>1$ resource blocks, a certain level of coordination is required in the system, as the transmitted binary codewords by the individual users should be reconstructed from the signals received over the $\rho$ resource blocks. To enable decoding, we divide the $V$ resource blocks in groups of $\rho$ resource blocks each, and the total number of users $\Ktot$ into $V/\rho$ groups of size $L=\Ktot\rho/V$. The $L$ users from the same group are configured to share the same $\rho$ resource blocks and the decoder operates over each group independently. 
%A user-error is declared if the message of a user is not contained in the output list. 

\subsubsection{AWGN channel}
Fig.~\ref{fig:unsourced_100_bits} illustrates the performance of the coding scheme from Section~\ref{sec:encoding_common_dictionary}, where a user message of size $b=98$ information bits is encoded over a block of $n$ channel uses (resource elements). We test two designs for the CW code that prescribes which columns of the dictionary matrix are combined to produce the transmit codeword. The first construction is obtained by concatenating a $\mathrm{PPM}(2^{14})$ code and a $\mathrm{RS}(11,7)$, resulting in a constant weight code with block size $N=11\cdot 2^{14}$. The dictionary matrix $\ACD\in\mathbb{C}^{n\times N}$ is obtained by taking $N=11\cdot 2^{14}$ sequences from the Gabor frame in dimension $n=431$  based on the Alltop construction described in Section~\ref{sec:dictionary_design}. 

The second construction is obtained by concatenating a $\mathrm{PPM}(2^{14})$ code and a $\mathrm{RS}(9,7)$, resulting in a constant weight code with block size $N=9\cdot 2^{14}$. The dictionary matrix $\ACD\in \mathbb{C}^{n\times N}$ is obtained by taking $N=9\cdot 2^{14}$ sequences from the Gabor frame in dimension $n=389$  based on the Alltop construction described in Section~\ref{sec:dictionary_design}.

We compare against the scheme based on the SPARCs construction from \cite{Fengler}, which applies the outer code from \cite{Amalladinne2018ACC}. We observe that, for a similar message size ($98$ bits vs $100$ bits in the example in \cite{Fengler}), the $E_b/{N_{0}}$ performance (for a reliability target $P_e=0.05$) of the coding approach proposed here is comparable, or improves over the approach in \cite{Fengler}, with the difference that this is achieved with a considerably smaller size of the transmitted codewords ($431$, i.e $389$ vs $30000$), which brings advantages in terms of transmission latency and/or bandwidth occupancy.

\begin{figure}[h!]
	\centering
	\includegraphics[width=.45\textwidth]{figures/100bits.png}
	\caption{Required $E_b/N_{0}$ for a target error probability $P_e=0.05$. AWGN channel.}
	\label{fig:unsourced_100_bits}
\end{figure}



In the following we present results for some parameterizations that we have observed to perform well in terms of the required $E_b/{N_0}$ for different message sizes.\smallskip

\textit{Message size $b=36$ bits:} The message is encoded over a single block of $n=149$ channel uses (resource elements). The CW code is obtained by concatenation of a $\mathrm{PPM}(2^{12})$ code and an $\mathrm{RS}(5,3)$ code. The dictionary matrix $\ACD\in \mathbb{C}^{n\times N}$ is obtained by taking $N=5\cdot 2^{12}$ sequences from the Gabor frame of dimension $n=149$  based on the Alltop construction.\smallskip

\textit{Message size $b=65$ bits:} The message is encoded over a single block of $n=257$ channel uses (resource elements). The CW code is obtained by concatenation of a $\mathrm{PPM}(2^{13})$ code and an $\mathrm{RS}(7,5)$ code. The dictionary matrix $\ACD\in\mathbb{C}^{n\times N}$ is obtained by taking $N=7\cdot 2^{13}$ sequences from the Gabor frame of dimension $n=257$ based on the Alltop construction.\smallskip

\textit{Message size $b=98$ bits:} The message is encoded over a single block of $n=389$ channel uses (resource elements). The CW code is obtained by concatenation of a $\mathrm{PPM}(2^{14})$ code and an $\mathrm{RS}(9,7)$ code. The dictionary matrix $\ACD\in \mathbb{C}^{n\times N}$ is obtained by taking $N=9\cdot 2^{14}$ sequences from the Gabor frame of dimension $n=389$ based on the Alltop construction.
\begin{figure}[h!]
	\centering
	\includegraphics[width=.45\textwidth]{figures/unsourced_nc_389_257_149.png}
	\caption{Required $E_b/N_{0}$ for a target error probability $P_e=0.05$. AWGN channel.}
	\label{fig:unsourced_389_257_149}
\end{figure}
We observe that, with the increase of the blocklength $n$, and thus with the message size that can be supported, the $E_b/{N_{0}}$ required to meet the reliability target $P_e=0.05$ decreases. For shorter message sizes, and hence shorter sequence lengths, on the other hand, we can serve more active users in the system at the cost of an increase of the required $E_b/{N_0}$ per user. 

\subsubsection{Block Rayleigh Fading Channel}
As described in Section \ref{sec:system_model}, we assume a Rayleigh block-fading model with coherence length no smaller than the block size $n$. We consider a non-coherent scenario, i.e. the fading realization in the block is unknown to both the transmitter and the receiver. We assume that the receiver has knowledge of the fading statistics, in this case the variance of the multiplicative Gaussian noise modelling Rayleigh fading.

In Fig.~\ref{fig:unsourced_fading_1} we assume transmission over a single fading block and plot the required $E_b/{N_{0}}$ as function of the number of active users $\Ka$ in the system, for message sizes $b=36$ and $b=65$ bits respectively. The block size $n$, the code parameterization and the choice of the Gabor dictionary matrices is the same as in the example in Fig.~\ref{fig:unsourced_389_257_149}. We perform simulations with $T=4$ and $T=8$ antennas at the receiver.
\begin{figure}[h!]
	\centering
	\includegraphics[width=.45\textwidth]{figures/multiantenna_unsourced.png}
	\caption{Required $E_b/N_{0}$ with multiple receive antennas, for a target error probability $P_e=0.05$. Block Rayleigh-fading channel.}
	\label{fig:unsourced_fading_1}
\end{figure}
In Fig.~\ref{fig:multiantenna_257} we depict the per-user probability of error $P_e$ as function of the $E_b/N_{0}$ for a message size $b=65$ bits. We assume transmission over a single block of length $n=257$, with the number of receive antennas $T\in\{2, 4, 8\}$ as parameter. We consider two different system loads (number of active users), $\Ka=466$ and $\Ka=1167$.  
\begin{figure}[h!]
	\centering
	\includegraphics[width=.45\textwidth]{figures/multiantenna_257.png}
	\caption{Probability of error $P_e$ vs. $E_b/N_{0}$, for different numbers of receive antennas $T$. Block Rayleigh fading channel.}
	\label{fig:multiantenna_257}
\end{figure}

\subsection{Separate Dictionaries}
As described in Section~\ref{sec:separate_dictionaries}, in this scenario the users employ a separate (i.e. user-specific) dictionary matrix to map their binary codewords on the channel resources. 
%In practice, this scheme can be implemented by \textit{configuring} $L$ users to share $v$ resource blocks, where $\rho\leq v\leq V$, and assigning each of the $L$ users a separate dictionary matrix $\mathbf{A}_i\in\mathbb{C}^{n\times N}$, $i\in\I$. Under these assumptions, the total number of users that can be configured on the $V$ resource blocks is $\Ktot=L V/v$.

\subsubsection{AWGN Channel}
In Fig.~\ref{fig:unsourced_vs_sourced_36bits} we provide a performance comparison between the approach based on a common dictionary (i.e. unsourced access scenario) and the approach based on separated dictionaries, in the following also referred to as "sourced" access scenario. We fix the message size to be $b=36$ bits in both scenarios. The user messages are encoded over a block of $n=257$ channel uses (resource elements). 

For the unsourced access scenario we use a CW code obtained by a concatenation of a $\mathrm{PPM}(2^{12})$ and an $\mathrm{RS}(7,3)$ Reed-Solomon code. The dictionary matrix $\ASD\in\mathbb{C}^{n\times N}$, which is shared among the users in the unsourced scenario, is obtained by taking $N=7\cdot 2^{12}$ sequences from the $n=257$-dimensional Gabor frame based on the Alltop construction described in Section~\ref{sec:dictionary_design}. 

For the "sourced" access scenario we use the same $n=257$-dimensional Gabor frame, with the difference that the $257\times 257^{2}$ Gabor matrix is  divided into $257$ sections of size $257$ sequences each, as given by  \eqref{eq:Gabor_frame} and \eqref{eq:Alltop_seed}. 

When $L\leq 257$ users in total are configured on the resource block of size $257$ channel uses, the $l$-th user ($1\leq l \leq L)$ is assigned the $l$-the section of the Gabor matrix. 

We take the first $15\cdot 16=240$ sequences from the section to obtain the dictionary matrix $\ASD_l\in \mathbb{C}^{257\times 240}$ that is used to map the user's message on the resource block of size $n=257$ resource elements. 

For the "sourced" access scenario we evaluate the performance as function of the number of system users $L$  configured on the same resource block of size $n=257$. We take $L=\{10, 20, 30, 40\}$ in the simulations. The total number of system users is then calculated as $\Ktot=L\ntot/n$. 
In both scenarios we assume $K=3$ active users within the resource block of size $n=257$, which gives in total $\Ka\approx350$ active users over the $\ntot=30000$ resources.
\begin{figure}[h!]
	\centering
	\includegraphics[width=.45\textwidth]{figures/unsourced_vs_sourced_3_users.png}
	\caption{Performance comparison of "unsourced" and "sourced" random access in terms of error probability $P_e$ as function of  $E_b/N_{0}$. AWGN channel.}
	\label{fig:unsourced_vs_sourced_36bits}
\end{figure}
We observe that when the number of users $L$ configured on the same resource block of size $n=257$ is below $L=20$, corresponding to an overall number of system users $\Ktot\approx 2335$, the approach with separate dictionaries outperforms the approach with a common dictionary in terms of the required  $E_b/{N_{0}}$ to meet a target error probability  $P_e=0.05$. We observe that with a further increase of the $E_b/{N_{0}}$, the error probability of the unsourced approach decreases more steeply, eventually  outperforming the sourced approach for all tested values of $L$ (i.e. $\Ktot$). We note, however, that in the sourced access scenario, the use of separate dictionaries provides means for user identification, in contrast to the unsourced access scenario.   

\subsubsection{Rayleigh Fading Channel}
In Fig.~\ref{fig:unsourced_vs_sourced_36bits_2} we provide a performance comparison between the approach based on a common dictionary (unsourced access) and the approach based on separated dictionaries (sourced access). We fix the message size to be $b=36$ bits for the unsourced access scenario, and $b=36$ or $b=35$ bits in the sourced access scenario, depending on the code parameterization. The user messages are encoded over a single block of $n=149$ channel uses (resource elements). In both scenarios we consider a multiantenna receiver with $T=4$ receive antennas and $\Ka=6$ active users over the resource block of size $n=149$ resources, i.e. $\Ka\approx 1208$ active users in total over the $\ntot=30000$ resources. 

For the unsourced access scenario we use a CW code obtained by a concatenation of a $\mathrm{PPM}(2^{12})$ and an $\mathrm{RS}(5,3)$ Reed-Solomon code. The dictionary matrix $\ASD\in \mathbb{C}^{n\times N}$ is obtained by taking $N=5\cdot 2^{12}$ sequences from the $n=149$-dimensional Gabor frame based on the Alltop construction. 

For the sourced access scenario we use the same $n=149$-dimensional Gabor frame, with the difference that the Gabor matrix is divided into $L$ sections of size $\bar{N}$ sequences each (by discarding some of the $149^2$ sequences to fit the  dimension $\bar{N}L$, when necessary), where $L$ is the number of users configured on the resource block of size $149$ channel uses. The $l$-th user ($1\leq l \leq L)$ is assigned the $l$-the section of the Gabor matrix to serve as a unique dictionary $\ASD_l\in\mathbb{C}^{n\times \bar{N}}$. The $\bar{N}$ sequences of each of the users' dictionaries are further divided into blocks (subsections) of size $M$. For the "sourced" access scenario we evaluate the performance for different numbers of system users $L$  configured on the same resource block of size $n=149$ channel uses. In the following, we consider only an inner $\mathrm{PPM}(M)$ code (without and RS outer code), with the following parameterization:
\begin{enumerate}
    \item $\mathrm{PPM}(2^9)$, $\bar{N}=4\cdot 2^9$ ($4$ information symbols corresponding to a message size $b=36$ bits), $L=10$ users configured on the resource block (corresponding to $\Ktot\approx 2014$).
    \item $\mathrm{PPM}(2^7)$, $\bar{N}=5\cdot 2^7$ ($5$ information symbols corresponding to a message size $b=35$ bits), $L=34$ users configured on the resource block (corresponding to $\Ktot\approx 6846$).
    \item $\mathrm{PPM}(2^6)$, $\bar{N}=6\cdot 2^6$ ($6$ information symbols corresponding to a message size $b=36$ bits), $L=57$ users configured on the resource block (corresponding to $\Ktot\approx 11477$).
    \item $\mathrm{PPM}(2^5)$, $\bar{N}=7\cdot 2^5$ ($7$ information symbols corresponding to a message size $b=35$ bits), $L=99$ users configured on the resource block (corresponding to $\Ktot\approx 19933$).
    \item $\mathrm{PPM}(2^4)$, $\bar{N}=9\cdot 2^4$ ($9$ information symbols corresponding to a message size $b=36$ bits), $L=154$ users configured on the resource block (corresponding to $\Ktot\approx 31007$).
\end{enumerate}

\begin{figure}[h!]
	\centering
	\includegraphics[width=.45\textwidth]{figures/unsourced_vs_sourced_6_users_multiantenna.png}
	\caption{Performance comparison of "unsourced" and "sourced" random access in terms of error probability $P_e$ as function of  $E_b/N_{0}$. Rayleigh Fading Channel. $T=4$ receive antennas.}
	\label{fig:unsourced_vs_sourced_36bits_2}
\end{figure}

We observe that when the number of users $L$ configured on the same resource block of size $n=149$ is below $L=34$, corresponding to an overall number of system users $\Ktot\approx 6846$, the approach with separate dictionaries outperforms the approach with a common dictionary in terms of the required  $E_b/{N_{0}}$ to meet a target error probability $P_e=0.05$. With increasing $L$ beyond this value, the unsourced approach performs better. As before, we note that in the sourced access scenario, the use of separate dictionaries provides in addition means for user identification, in contrast to the unsourced access scenario.

==> sections/review_questions.tex <==
\section{Editor's Comments}
\textcolor{black}{
\begin{enumerate}
    \item The contribution of the paper is not clear compared to existing works in the literature, as pointed out by the reviewers. 
    \item The authors should provide some justifications for the adopted system model. Also, please discuss the possibility of extending the current results to the case of wideband frequency selective channels. 
    \item The complexity of the code design should be discussed. 
    \item The use of AMP-type decoder should be justified as it may not work well in some situations.
    \item The authors should provide more discussions on the simulation results. 
\end{enumerate}
}



==> sections/system_model_old.tex <==
\section{System Model and Encoding} \label{sec:system_model}

\subsection{System Model}

Consider a multiple access channel where communication is performed over $\bar{n}$ channel uses. We assume a pool of $K$ possible users indexed by the set $\mathcal{I}:=\{1,\dots,K\}$, that can transmit over the $\bar{n}$ channel uses. We furthermore denote by $\mathcal{I}_{\mathrm{a}}\subseteq\mathcal{I}$ the set of active users of cardinality $\vert\mathcal{I}_{\mathrm{a}}\vert=K_{\mathrm{a}}$. The activity of every user $i\in\mathcal{I}$ is captured by the random variable $\mathrm{\lambda}_i\in\{0,1\}$, with $\lambda_i=1$ if $i\in\mathcal{I}_{\mathrm{a}}$, and $\lambda_i=0$ otherwise. The $\bar{n}$ channel resources are split over $V$ (resource) blocks, each of size $n=\bar{n}/V$. 

When active, user $i$ selects a message $W_i$ of size $L\log_2 M$ bits from its transmit buffer and spreads it over $\rho$ such blocks, $1\leq\rho\leq V$, by generating a transmit vector (transmit codeword) $\mathbf{s}_i=[\mathbf{s}_{i}^{(1)};\ldots;\mathbf{s}_{i}^{(\rho)}]\in\mathbb{C}^{n\rho}$, where $\mathbf{s}_{i}^{(1)}, \ldots, \mathbf{s}_{i}^{(\rho)}\in\mathbb{C}^{n}$ are the sub-vectors of $\mathbf{s}_i$ transmitted respectively in each of the $\rho$ resource blocks, and we further assume that all users $i\in\mathcal{I}$ are subject to the same power constraint $\mathbb{E} {\Vert\mathbf{s}_i\Vert^2}\doteq E_s=\rho n P$. 

Without loss of generality, in the following we describe the system model for the first of the $V$ blocks of size $n$. Let $\mathbf{y}_1\in\mathbb{C}^{n}$ and $\mathbf{z}_1\in\mathbb{C}^{n}$ be the vectors of channel outputs and channel noise, respectively, of the first block. Assuming a block-fading model with coherence time-frequency span no smaller than the block size $n$, the received signal over the first block reads
\begin{equation}
	\mathbf{y}_1 = \sum\limits_{i\in\mathcal{I}_{\mathrm{a}}}h_{i}^{(1)}\mathbf{s}_{i}^{(1)}+\mathbf{z}_1, \label{eq:system_model}
\end{equation} 
where $\mathbf{s}_{i}^{(1)}$ is the part (i.e. sub-vector) of the transmit vector $\mathbf{s}_{i}$ of the active user $i\in\mathcal{I}_{\mathrm{a}}$ transmitted over the first block, and $h_{i}^{(1)}$ is the channel coefficient for the wireless channel between user $i$ and the receiver for the first resource block. The entries of the noise vector $\mathbf{z}_1$ are i.i.d. complex Gaussian with zero mean and variance $N_0$. With this, the user signal-to-noise ratio is $\mathrm{SNR}=\frac{E_s}{\rho n N_0}=\frac{P}{N_{0}}$. 
We consider a \textit{non-coherent} communication scenario, i.e. we drop the assumption of \textit{a priori} channel state information (CSI) at the transmitter and at the receiver side, and instead assume that the receiver knows only the statistics of the fading process. 

\subsection{Encoding}
The encoding procedure is as follows. Each active user $i\in\mathcal{I}_{\mathrm{a}}$ first splits its transmit message $W_i$ into $L$ chunks of size $\log_2 M$ bits. We denote by $e_i^{(l)}\in\mathbb{F}_{M}$ the Galois field representation of these chunks which give rise to the indices of the sequences to be sent from the corresponding codebook sections $l\in\vert L\vert$. Let $g:\mathbb{F}_{M}\rightarrow \{0,1\}^{M}$ denote a $1$-of-$M$ encoder \cite{bishop1}, the resulting selection indices can be represented in binary vector form $\mathbf{c}_i=[g(e_i^{(1)});\dots;g(e_i^{(L)})]\in\{0,1\}^N$. The resulting binary vector is then mapped to a vector
\begin{equation}
    \mathbf{s}_i=\bar{\mathbf{A}}_i\mathbf{c}_i\label{eq:dictionary_mapping}
\end{equation}
of length $n\rho$ by a matrix $\bar{\mathbf{A}}_l=\mathbf{I}_{\rho}\otimes\mathbf{A}_l\in\mathbb{C}^{n\rho\times N \rho}$ and transmitted over the $\bar{n}=n\rho$ channel resources (i.e. over the $\rho$ resource blocks of size $n$). The product is properly scaled such as to fulfil the average power constraint $\mathbb{E}\Vert\mathbf{s}_l\Vert =\rho nP$. The matrix $\bar{\mathbf{A}}_l$ is block-diagonal where each block contains the same smaller matrix $\mathbf{A}_l\in\mathbb{C}^{n\times N}$. The matrices $\mathbf{A}_l$, $l=1,\ldots,K$ can be interpreted as user dictionaries whose columns are (complex-valued) sequences of dimension $n$. 
%The binary vector $\mathbf{c}_l=[\mathbf{c}_{l}^{(1)};\ldots; \mathbf{c}_{l}^{(\rho)}]$, whose sub-vectors $\mathbf{c}_{l}^{(1)}, \ldots, \mathbf{c}_{l}^{(\rho)}\in \mathbb{F}_2^{\bar{n}}$ are mapped on the $\rho$ resource blocks via \eqref{eq:dictionary_mapping}, prescribes which  sequences from the dictionary $\bar{\mathbf{A}}_l$ are combined in each resource block to produce the transmit vector $\mathbf{s}_l$.  
Depending on the structure of the dictionary matrices $\mathbf{A}_l$, we will distinguish between the following approaches. 

\subsubsection{Common Dictionary (CD)}\label{sec:common_dictionary}
According to this approach, all users employ a common (i.e. a shared) dictionary  $\mathbf{A}_i=\mathbf{A}$, $i\in\mathcal{I}$, to map their codewords $\mathbf{c}_i$ on the $\rho$ resource blocks. Following \eqref{eq:system_model}, the signal received over the first resource block reads  
\begin{align}
    \mathbf{y}_1 &= \bar{\mathbf{A}}\sum\limits_{i\in\mathcal{I}_{\mathrm{a}}} h_i^{(1)}\mathbf{c}_i^{(1)}+\mathbf{z}_1. \label{eq:CD}
\end{align}
By defining
\begin{equation}
    \mathbf{x}_1=\sum\limits_{i\in\mathcal{I}_{\mathrm{a}}} h_i^{(1)}\mathbf{c}_i^{(1)},
\end{equation}
\eqref{eq:CD} can be further written in a more compact form as 
\begin{align}
    \mathbf{y}_1=\bar{\mathbf{A}}\mathbf{x}_1 + \mathbf{z}_1.   
\end{align} 
This approach is well suited to the unsourced random access model in \cite{polyanskiy17}, \cite{ordentlich17} which decouples the user identification problem and the data transmission problem. In that case, the role of the decoder is to output a list $\mathcal{L}(y)=\{W_1,\ldots,W_J\}\subset[M]^J$ of no more than $K_{\mathrm{a}}$ messages ($J\leq K_{\mathrm{a}})$ that should contain most messages that were transmitted by the active users, where the order in which the messages appear in the list is of no significance. In other words, the decoder only declares which messages were transmitted, without associating the messages to the users that transmitted them. With this approach, the decoder's error probability is defined as
% \begin{equation}
%     P_{\mathrm{e}}=\max\limits_{\vert\boldsymbol{\lambda}\vert=K_{\mathrm{a}}}\frac{1}{K_{\mathrm{a}}}\sum_{i\in\mathcal{I}_{\mathrm{a}}}\lambda_i\cdot\mathbb{P}\left(W_i\notin \mathcal{L}(\mathbf{y})\right),
%     \label{eq:decoding_error_JC}
% \end{equation}
\begin{equation}
    P_{\mathrm{e}}=\frac{1}{K_{\mathrm{a}}}\sum_{i\in\mathcal{I}_{\mathrm{a}}}\mathbb{P}\left(W_i\notin \mathcal{L}(\mathbf{y})\right).
    \label{eq:decoding_error_JC}
\end{equation}
We note that this formulation requires that the number of active users $K_{\mathrm{a}}$ is \textit{known} to the decoder. As a consequence, the parameter $K$ (the total number of users in the system) does not affect the error probability, and can thus be left out of the model (i.e. it can be set to $\infty$). 

We remark that, although the random access model is unsourced, in the case when the active users spread their messages over $\rho>1$ resource blocks, a certain level of coordination is required in the system, as the transmitted binary codewords should be reconstructed from the signals received over the $\rho$ resource blocks. To enable decoding in this case, one can for example divide the total number of users $K$ into $V/\rho$ groups of size $L=K\rho/V$, where the $L$ users from the same group are configured to share the same $\rho$ resource blocks. 

\subsubsection{Separate Dictionaries (SD)} \label{sec:separate_dictionaries}

According to this approach, the users employ a separate (i.e. user-specific) dictionary matrix to map their binary codewords $\mathbf{c}_i$ on the channel resources. In practice, this scheme can be implemented by \textit{configuring} $K'$ users to share $v$ resource blocks, where $\rho\leq v\leq V$, and assigning each of the $K'$ users a separate dictionary matrix $\mathbf{A}_i\in\mathbb{C}^{n\times N}$, $i=1,\ldots, L$. We remark that, under these assumptions, the total number of users that can be configured on the $V$ resource blocks is $K=LV/v$.   

With this, based on \eqref{eq:system_model}, the signal received over the first resource block can be written as
\begin{align}
    \mathbf{y}_1 &= \sum\limits_{j=1}^L
    \lambda_{i_j}h_{i_j}^{(1)}\bar{\mathbf{A}}_{j}\mathbf{c}_{i_j}^{(1)}+\mathbf{z}_1, \label{eq:SD}
\end{align}
where $i_1,\ldots, i_L$ are the indices of the $L$ users configured on the first resource block. By defining $\bar{\mathbf{A}}=\left[\bar{\mathbf{A}}_1, \ldots, \bar{\mathbf{A}}_L\right]\in\mathbb{C}^{\bar{n}\times NL}$ to be the matrix that concatenates the $L$ dictionary matrices, \eqref{eq:SD} can be further written in a more compact form as
\begin{equation}
    \mathbf{y}_1=\bar{\mathbf{A}}\mathbf{x}_1+\mathbf{z}_1, \label{eq:separate_dictionaries}
\end{equation}
where we have defined $\mathbf{x}_1=\Gamma_1 \mathbf{c}_1\in \mathbb{C}^{NL\times 1}$. Here $\Gamma_1$ is a $NL\times NL$ diagonal matrix that has $[\gamma_{i_1}\mathbf{1}, \ldots, \gamma_{i_L}\mathbf{1}]$ on the main diagonal, where $\gamma_{i_j}=\lambda_{i_j}h_{i_j}$, and $\mathbf{1}$ is an all-one vector of corresponding dimension (here $N$). The binary vector $\mathbf{c}_1\in \mathbb{F}_2^{N L}$ stacks the binary vectors $\mathbf{c}_{i_j}^{(1)}$ from the individual users, $\mathbf{c}_1=[\mathbf{c}_{i_1}^{(1)}; \ldots ; \mathbf{c}_{i_L}^{(1)}]$.




==> tikz/factorgraph.tex <==
\tikzset{
  vn/.style = {draw,minimum width=1.75em, shape=circle,thick, black,fill=white,inner sep=0pt},
  fn/.style ={draw, minimum height=1.5em, minimum width=1.5em, shape=rectangle,thick, black,fill=black},
  ffn/.style ={draw, minimum height=10em, minimum width=1.5em, shape=rectangle,thick, black,fill=black},
  none/.style ={draw=none, minimum height=2em, minimum width=2em, shape=rectangle},
  plate/.style={draw,
    shape=rectangle,
    thick,
    minimum width=4em,
    minimum height=4em,
    align=right,
    inner sep=5em,
    inner ysep=5em,
    label={[xshift=-16pt,yshift=11pt]south east:#1}},
  line/.style={draw, -},
  jump left/.style={draw=none, inner xsep=0pt},
  jump line/.style={line, shorten <=5pt}
}

\begin{tikzpicture}[auto,thick,node distance=5em]


\node[fn] (f1) {};
\node[fn, below of=f1,yshift=1em] (f2) {};
\node[fn, below of=f2,yshift=1em] (f3) {};

\node[fn, below of=f3,yshift=-3em] (f4) {};
\node[fn, below of=f4,yshift=1em] (f5) {};
\node[fn, below of=f5,yshift=1em] (f6) {};

\node[vn,left of=f1] (v1) {};
\node[vn,left of=f2] (v2) {};
\node[vn,left of=f3] (v3) {};
\node[vn,left of=f4] (v4) {};
\node[vn,left of=f5] (v5) {};
\node[vn,left of=f6] (v6) {};

\node[vn,right of=f1] (c1) {};
\node[vn,right of=f2] (c2) {};
\node[vn,right of=f3] (c3) {};
\node[vn,right of=f4] (c4) {};
\node[vn,right of=f5] (c5) {};
\node[vn,right of=f6] (c6) {};

\node[fn,right of=c1] (fc1) {};
\node[fn,right of=c2] (fc2) {};
\node[ffn,right of=c2] (fc22) {};
\node[fn,right of=c3] (fc3) {};

\node[fn,right of=c4] (fc4) {};
\node[fn,right of=c5] (fc5) {};
\node[ffn,right of=c5] (fc52) {};
\node[fn,right of=c6] (fc6) {};


\node[vn,right of=fc2] (l1) {};
\node[fn,right of=l1,xshift=-2em] (f7) {};
\node[vn,right of=fc5] (l2) {};
\node[fn,right of=l2,xshift=-2em] (f8) {};

\node[above of=c1,yshift=-3em] {$c_{11}$};
\node[above of=c2,yshift=-3em] {$c_{12}$};
\node[above of=c3,yshift=-3em] {$c_{1N}$};

\node[above of=c4,yshift=-3em] {$c_{L1}$};
\node[above of=c5,yshift=-3em] {$c_{L2}$};
\node[above of=c6,yshift=-3em] {$c_{LN}$};

\node[none,left of=v1] (cl1) {};\node[none,left of=v2] (cl2) {};\node[none,left of=v3] (cl3) {};
\node[none,left of=v4] (cl4) {};\node[none,left of=v5] (cl5) {};\node[none,left of=v6] (cl6) {};
\node[none,left of=cl6,xshift=-2em] (cl12) {};
\node[none,left of=cl5,xshift=-2em] (cl11) {};
\node[none,left of=cl4,xshift=-2em,yshift=-2.5em] (cl10) {};
\node[none,left of=cl3,xshift=-2em,yshift=-2.5em] (cl9) {};
\node[none,left of=cl2,xshift=-2em,yshift=-2.5em] (cl8) {};
\node[none,left of=cl1,xshift=-2em] (cl7) {};

\path [line] (f1) to (v1);%\path [line] (f1) to (v2);\path [line] (f1) to (v3);
\path [line] (f2) to (v2);%\path [line] (f2) to (v2);\path [line] (f2) to (v3);
\path [line] (f3) to (v3);%\path [line] (f3) to (v2);\path [line] (f3) to (v3);

\path [line] (f4) to (v4);%\path [line] (f4) to (v5);\path [line] (f4) to (v6);
\path [line] (f5) to (v5);%\path [line] (f5) to (v5);\path [line] (f5) to (v6);
\path [line] (f6) to (v6);%\path [line] (f6) to (v5);\path [line] (f6) to (v6);

\path [line] (f1) to (c1);%\path [line] (f1) to (v2);\path [line] (f1) to (v3);
\path [line] (f2) to (c2);%\path [line] (f2) to (v2);\path [line] (f2) to (v3);
\path [line] (f3) to (c3);%\path [line] (f3) to (v2);\path [line] (f3) to (v3);

\path [line] (f4) to (c4);%\path [line] (f4) to (v5);\path [line] (f4) to (v6);
\path [line] (f5) to (c5);%\path [line] (f5) to (v5);\path [line] (f5) to (v6);
\path [line] (f6) to (c6);%\path [line] (f6) to (v5);\path [line] (f6) to (v6);

\path [line] (fc4) to (c4);%\path [line] (f4) to (v5);\path [line] (f4) to (v6);
\path [line] (fc5) to (c5);%\path [line] (f5) to (v5);\path [line] (f5) to (v6);
\path [line] (fc6) to (c6);%\path [line] (f6) to (v5);\path [line] (f6) to (v6);

\path [line] (fc1) to (c1);%\path [line] (f4) to (v5);\path [line] (f4) to (v6);
\path [line] (fc2) to (c2);%\path [line] (f5) to (v5);\path [line] (f5) to (v6);
\path [line] (fc3) to (c3);%\path [line] (f6) to (v5);\path [line] (f6) to (v6);

\path [line] (f7) to (l1);
%\path [line] (fc1) to (l1);
\path [line] (fc2) to (l1);
%\path [line] (fc3) to (l1);

\path [line] (f8) to (l2);
%\path [line] (fc4) to (l2);
\path [line] (fc5) to (l2);
%\path [line] (fc6) to (l2);

\path [line] (v1) to (cl1);\path [line] (v2) to (cl2);\path [line] (v3) to (cl3);
\path [line] (v4) to (cl4);\path [line] (v5) to (cl5);\path [line] (v6) to (cl6);


\draw[draw=black] (cl1.north east) rectangle (cl12.south west);

\node[fn,left of=cl8] (f9) {};\node[vn,left of=f9,xshift=1.5em] (v9) {};
\node[fn,left of=cl9] (f10) {};\node[vn,left of=f10,xshift=1.5em] (v10) {};
\node[fn,left of=cl10] (f11) {};\node[vn,left of=f11,xshift=1.5em] (v11) {};

\path [line] (f9) to (v9);
\path [line] (f10) to (v10);
\path [line] (f11) to (v11);

\path [line] (cl8) to (f9);
\path [line] (cl9) to (f10);
\path [line] (cl10) to (f11);


\node[left of=v9,xshift=3em] {$\mathbf{y}_1$};
\node[left of=v10,xshift=3em] {$\mathbf{y}_2$};
\node[left of=v11,xshift=3em] {$\mathbf{y}_{\bar n}$};

\node[above of=f9,yshift=-3em] {$P\left(\mathbf{y}_1\vert \mathbf{z}_1\right)$};
\node[above of=f10,yshift=-3em] {$P\left(\mathbf{y}_2\vert \mathbf{z}_2\right)$};
\node[above of=f11,yshift=-3em] {$P\left(\mathbf{y}_{\bar n}\vert \mathbf{z}_{\bar n}\right)$};


\node[above of=v1,yshift=-3em] {$\mathbf{x}_{11}$};
\node[above of=v2,yshift=-3em] {$\mathbf{x}_{12}$};
\node[above of=v3,yshift=-3em] {$\mathbf{x}_{1N}$};

\node[above of=v4,yshift=-3em] {$\mathbf{x}_{L1}$};
\node[above of=v5,yshift=-3em] {$\mathbf{x}_{L2}$};
\node[above of=v6,yshift=-3em] {$\mathbf{x}_{LN}$};

\node[right of=f7,xshift=-2.5em] {$p\left(\lambda_1\right)$};
\node[right of=f8,xshift=-2.5em] {$p\left(\lambda_L\right)$};

\node[above of=fc1,yshift=-2.5em] {$p\left(\mathbf{c}_1\vert\lambda_1\right)$};
\node[above of=fc4,yshift=-2.5em] {$p\left(\mathbf{c}_L\vert\lambda_L\right)$};

\node[above of=l1,yshift=-3em] {$\lambda_1$};
\node[above of=l2,yshift=-3em] {$\lambda_L$};

\node[above of=f1,yshift=-3em] {$p\left(\mathbf{x}_{11}\vert c_{11}\right)$};
\node[above of=f2,yshift=-3em] {$p\left(\mathbf{x}_{12}\vert c_{12}\right)$};
\node[above of=f3,yshift=-3em] {$p\left(\mathbf{x}_{1N}\vert c_{1N}\right)$};

\node[above of=f4,yshift=-3em] {$p\left(\mathbf{x}_{L1}\vert c_{L1}\right)$};
\node[above of=f5,yshift=-3em] {$p\left(\mathbf{x}_{L2}\vert c_{L2}\right)$};
\node[above of=f6,yshift=-3em] {$p\left(\mathbf{x}_{LN}\vert c_{LN}\right)$};

\node[right of=cl9,xshift=-1.5em,yshift=-1em](cl9) {\huge$\mathbf{A}$};

\node[below of=v10,yshift=2em](dot) {\large$\vdots$};
\node[right of=dot](dot) {\large$\vdots$};
\node[below of=v3,yshift=2em] {\large$\vdots$};
\node[below of=f3,yshift=2em] {\large$\vdots$};
\end{tikzpicture}




==> tikz/matrix.tex <==
% \tikzset{
%     ncbar angle/.initial=90,
%     ncbar/.style={
%         to path=(\tikztostart)
%         -- ($(\tikztostart)!#1!\pgfkeysvalueof{/tikz/ncbar angle}:(\tikztotarget)$)
%         -- ($(\tikztotarget)!($(\tikztostart)!#1!\pgfkeysvalueof{/tikz/ncbar angle}:(\tikztotarget)$)!\pgfkeysvalueof{/tikz/ncbar angle}:(\tikztostart)$)
%         -- (\tikztotarget)
%     },
%     ncbar/.default=0.5cm,  
% }
% \tikzset{square left brace/.style={ncbar=0.20cm}}
% \tikzset{square right brace/.style={ncbar=-0.2cm}}
\begin{tikzpicture}

\matrix (m) [matrix of math nodes, nodes in empty cells,every node/.style={anchor=base,align=left,text depth=.8em,text height=.8em,text width=1.5em},
inner sep=0pt, column sep=0.3em, row sep=0.1em]{
    &   &   &   &   & &   &   &   &  &  &  &  &  &  &  &  &  &&&&\\
 &   &   &   &   & &   &   &   &  &  &  &  &  &  &  &  &  &&&&\\
 &   &   &   &   & &   &   &   &  &  &  &  &  &  &  &  &  &&&&\\
 &   &   &   &   & &   &   &   &  &  &  &  &  &  &  &  &  &&&&\\
 &   &   &   &   & &   &   &   &  &  &  &  &  &  &  &  &  &&&&\\
 &   &   &   &   & &   &   &   &  &  &&& & & & & &&&&\\
 &   &   &   &   & &   &   &   &  &  &  &  &  &  &  &  &  &&&&\\
 &   &   &   &   & &   &   &   &  &  &  &  &  &  &  &  &  &&&&\\
 &   &   &   &   & &   &   &   &  &  &  &  &  &  &  &  &  &&&&\\
 &   &   &   &   & &   &   &   &  &  &  &  &  &  &  &  &  &&&&\\%
 &   &   &   &   & &   &   &   &  &  &  &  &  &  &  &  &  &&&&\\
 &   &   &   &   & &   &   &   &  &  &  &  &  &  &  &  &  &&&&\\
 & 0 & 0 & 0  & 1  &0 & 0  & 0  &  1 & 0 & 0 &  &  &  & 0 & 1 & 0 & 0 &0&&&\\
 &   &   &   &   & &   &   &   &  &  &  &  &  &  &  &  &  &&&&\\
};

% % Strich 

\draw [thick] (m-2-2.north west) to [square right brace ] (m-9-2.south west);
\draw [thick] (m-2-19.north east) to [square left brace ] (m-9-19.south east);

\draw [thick] (m-12-2.west) to [square right brace ] (m-13-2.south west);
\draw [thick] (m-12-19.east) to [square left brace] (m-13-19.south east) ;
 
\draw[] (m-2-6.north east) -- (m-9-6.south east);
\draw[] (m-2-11.north east) -- (m-9-11.south east);
\draw[] (m-2-14.north east) -- (m-9-14.south east);

\draw[] (m-12-6.east) -- (m-13-6.south east);
\draw[] (m-12-11.east) -- (m-13-11.south east);
\draw[] (m-12-14.east) -- (m-13-14.south east);

\node[above=1pt,xshift=.1cm,yshift=-.15cm] at (m-5-13.south west) {$\cdots$} ;
\node[above=1pt,yshift=-.1cm,xshift=.3cm] at (m-13-12.east) {$\cdots$} ;

\node[xshift=-.75cm] at (m-5-1.south) {\begingroup\fontsize{18pt}{18pt}$\mathbf{A}:=$\endgroup};
\node[xshift=-.75cm,yshift=.1cm] at (m-13-1) {\begingroup\fontsize{18pt}{18pt}$\mathbf{c}^T:=$\endgroup};

% \node[] at (m-5-22.south) {\begingroup\fontsize{18pt}{18pt}$\large\in\mathbb{C}^{N\times ML}$\endgroup};

\draw[<->,thick] (m-1-1) --node[above=1pt] {$M$} (m-1-6.east);
\draw[<->,thick] (m-1-6.east) --node[above=1pt] {$M$} (m-1-11.east);
\draw[<->,thick] (m-1-14) --node[above=1pt] {$M$} (m-1-19.east);
\draw[<->,thick] (m-1-20.south east) --node[right=1pt] {$\blck$} (m-10-20.north east);

\draw[decorate,decoration={brace,amplitude=4pt,mirror}] (m-14-1) -- node[below=2pt] {$\mathbf
{c}^{(1)}$}(m-14-6.east); 
\draw[decorate,decoration={brace,amplitude=4pt,mirror}] (m-14-6) -- node[below=2pt] {$\mathbf
{c}^{(2)}$}(m-14-11.east); 
\draw[decorate,decoration={brace,amplitude=4pt,mirror}] (m-14-14) -- node[below=2pt] {$\mathbf
{c}^{(L)}$}(m-14-19.east); 



\draw[color=white,fill=gray, fill opacity=0.2] (m-2-5.north west) rectangle (m-9-5.south);
\draw[color=white,fill=gray, fill opacity=0.2] (m-2-16.north west) rectangle (m-9-16.south);
\draw[color=white,fill=gray, fill opacity=0.2] (m-2-9.north west) rectangle (m-9-9.south);


\end{tikzpicture}

